Eigenstate Thermalisation on Average

We consider conditions under which an isolated quantum system approaches a microcanonical equilibrium state. A key component is the eigenstate thermalisation hypothesis, which proposes that all energy eigenstates appear thermal. We introduce a weaker version of this requirement, applying only to the average distinguishability of eigenstates from the thermal state, and investigate its necessity and sufficiency for thermalisation.

==> theorems/thm2_degeneracies.tex <==
Consider an energy band of overall dimension $d$, which contains $d'$ distinct energy levels characterised by the projectors $\{\Pi_i\,:\,i=1,...,d'$\}. Let each energy level have degeneracy $g(i)$ such that $\sum_{i=1}^{d'} g(i) = d$.

Let $\mathcal{B} = \{\rho_n^i\,:\,i=1,...,d';\,n=1,...,g(i)\}$ be the orthonormal energy basis which maximises mean distinguishability from the microcanonical state, as in equation D6. Without loss of generality, assume that in each degenerate level, $\DEm{\rho_1^i,\Omega}\geq\DEm{\rho_n^i,\Omega}$ for $n>1$.

It follows from equations B1-B6 that there must exist some time-averaged state $\omega'\in\mathrm{span}\{\rho^1_1,...,\rho^{d'}_1\}$ with effective dimension no less that $\frac{d'}{4}$ such that
\begin{equation}
    \DEm{\omega',\Omega'}\geq \frac{1}{N_{\mathcal{M}}}\cdot\frac{1}{d'}\sum_{i=1}^{d'} \DEm{\rho_1^i,\Omega'},
\end{equation}
where $\Omega'=\frac{1}{d'}\sum_{i=1}^{d'} \rho_1^i$.
